Software Citation in HEP: Current State and Recommendations for the Future

In November 2022, the HEP Software Foundation and the Institute for Research and Innovation for Software in High-Energy Physics organized a workshop on the topic of Software Citation and Recognition in HEP. The goal of the workshop was to bring together different types of stakeholders whose roles relate to software citation, and the associated credit it provides, in order to engage the community in a discussion on: the ways HEP experiments handle citation of software, recognition for software efforts that enable physics results disseminated to the public, and how the scholarly publishing ecosystem supports these activities. Reports were given from the publication board leadership of the ATLAS, CMS, and LHCb experiments and HEP open source software community organizations (ROOT, Scikit-HEP, MCnet), and perspectives were given from publishers (Elsevier, JOSS) and related tool providers (INSPIRE, Zenodo). This paper summarizes key findings and recommendations from the workshop as presented at the 26th International Conference on Computing in High Energy and Nuclear Physics (CHEP 2023).

==> Makefile <==
FILENAME = chep_2023_proceedings

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

LATEX = lualatex

BIBTEX = bibtex

default: document copy_draft

all: default

figures: $(figure_list)

figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

document: figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn *.pyg

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: deep_clean text
	
	sed -i.bak 's/cache=false/cache=true/' latex/packages.tex
	$(MAKE) text

	mkdir submit_to_arXiv
	cp $(FILENAME).tex submit_to_arXiv
	if [ -f $(FILENAME).bbl ]; then cp $(FILENAME).bbl submit_to_arXiv/ms.bbl; fi
	cp Makefile submit_to_arXiv

	if [ -d src ]; then cp -r src submit_to_arXiv; fi
	if [ -d latex ]; then cp -r latex submit_to_arXiv; fi
	if [ -d figures ]; then cp -r figures submit_to_arXiv; fi
	if [ -f *.sty ]; then cp *.sty submit_to_arXiv; fi
	
	if [ -f *.bst ]; then cp *.bst submit_to_arXiv; fi
	
	if [ -f 00README.XXX ]; then cp 00README.XXX submit_to_arXiv; fi

	
	
	mv _minted-$(FILENAME) submit_to_arXiv/_minted-ms
	sed -i.bak 's/finalizecache/frozencache/' submit_to_arXiv/latex/packages.tex

	mv submit_to_arXiv/$(FILENAME).tex submit_to_arXiv/ms.tex

	
	
	sed -i.bak '/^ *

	
	
	

	find submit_to_arXiv/ -name "*.bak" -type f -delete

	
	find submit_to_arXiv/ -name "*.bib" -type f -delete

	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean

	
	if [ -f latex/packages.tex.bak ];then \
		mv latex/packages.tex.bak latex/packages.tex; \
	fi

list_arXiv:
	tar -tvf submit_to_arXiv.tar.gz

test_arXiv:
	tar -xzvf submit_to_arXiv.tar.gz
	cd submit_to_arXiv && make

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv


==> latex/packages.tex <==
\usepackage[varg]{txfonts}   % Web of Conferences font
\usepackage{amsmath,bm}
\usepackage{hyperref}
\graphicspath{{figures/}}
\usepackage{listings}  % Need verbatim for PYTHIA banner
\RequirePackage{caption}
\usepackage[cache=true,newfloat=true,frozencache]{minted}
\usepackage[capitalize]{cleveref}% https://ctan.org/pkg/cleveref % Must be loaded after hyperref
\usepackage{orcidlink}

\usemintedstyle{friendly}
\setminted[yaml]{fontsize=\scriptsize, numbersep=5pt, framesep=2mm, gobble=0}
\captionsetup[listing]{skip=-5pt}

\hypersetup{bookmarksnumbered=true, bookmarksopen=true, bookmarksopenlevel=0}
\hypersetup{pdftitle={Software Citation in HEP: Current State and Recommendations for the Future}, pdfauthor={Feickert, Katz, Neubauer, Sexton-Kennedy, Stewart}}
\hypersetup{colorlinks,breaklinks}
\hypersetup{linkcolor=blue,citecolor=blue,filecolor=black,urlcolor=blue}

